GentleRain+: Making GentleRain Robust on Clock Anomalies

Causal consistency is in an intermediate consistency model that can be achieved together with high availability and high performance requirements even in presence of network partitions. There are several proposals in the literature for causally consistent data stores. Thanks to the use of single scalar physical clocks, GentleRain has a throughput higher than other proposals such as COPS or Orbe. However, both of its correctness and performance relay on monotonic synchronized physical clocks. Specifically, if physical clocks go backward its correctness is violated. In addition, GentleRain is sensitive on the clock synchronization, and clock skew may slow write operations in GenlteRain. In this paper, we want to solve this issue in GenlteRain by using Hybrid Logical Clock (HLC) instead of physical clocks. Using HLC, GentleRain protocl is not sensitive on the clock skew anymore. In addition, even if clocks go backward, the correctness of the system is not violated. Furthermore, by HLC, we timestamp versions with a clock very close to the physical clocks. Thus, we can take causally consistency snapshot of the system at any give physical time. We call GentleRain protocol with HLCs GentleRain+. We have implemented GentleRain+ protocol, and have evaluated it experimentally. GentleRain+ provides faster write operations compare to GentleRain that rely solely on physical clocks to achieve causal consistency. We have also shown that using HLC instead of physical clock does not have any overhead. Thus, it makes GentleRain more robust on clock anomalies at no cost.

==> protocol__mohammad_roohitavaf_s_conflicted_copy_2016-08-19_.tex <==
\section{MSU-DB Protocol}

The MSU-DB protocol is similar to GentleRain protocol in many aspects. The main difference between MSU-DB and GentleRain is using HLC instead of physical clock for timestamping versions.

\subsection{Client Side}
In this section we focus on the client side of the protocol. The client states and operations in the MSU-DB is the same as those in the GentleRain. Table \ref{??} shows two variables that define the state for a client. $DT_c$ is the maximum HLC timestampt of an item accessed by client $c$. As discussed in Section \ref{??}, both GentleRain and MSU-DB maintains a variable called Global Stable Time (GST) in each data center such that condition $I2$ defined in Section \ref{??} is satisfied at all time. Each client maintain the most updated value of the GST of its corresponding data center. When a server processes a client request, it returns the $GST$ back to the client. Client stores GST value returned from the server in its $GST_c$ variable.


\begin{center} 
\begin{table} [h]
\caption{Variables maintained by client $c$}
\begin{tabular}{ |l|l|l| } 

\hline
\textbf{Variable} & \textbf{Definition} \\
\hline
$DT_c$ & dependency time at client $c$ \\ 
$GST_c$ & global stable time known by client $c$ \\ 
\hline
\end{tabular}
\end{table}
\end{center}

Algorithm \ref{alg:client} shows the two operations that a client can perform on the system. When a client wants to read the value of an item, it sends a $\textsc{GetReq}$ message to the server maintaining the item. In addition to the key of the item, the client also piggybacks the value of its $GST_c$ to the message. The server uses this value of update it own GST. Client then wait to receive the reply from the server. In the $\textsc{GetReply}$ message, the server sends the value of the requested item back to the client. The server also piggybacks the value of its GST and the timestamp of the value. We will discuss how the server find the correct version of an item to send to the client in Section \ref{??}. Upon receiving $\textsc{GetReply}$ message, the client update its dependency time $DT_c$ to timestamp of the returned value if the latter is larger than the current $DT_c$. Similarly, the client update its $GST_c$ if the $gst$ value returned by the server is higher. Note that $DT_c$ and $GST_c$ are HLC values, so the comparisons for computing the maximum of values are done as discussed in Section \ref{??}.

\begin{algorithm} 
{
\caption{Client operations at client $c$.}
\label{alg:client}
\begin{algorithmic} [1]

%\STATE // 
%\STATE 
\STATE \textbf{GET} (key $k$) %\COMMENT{ }

\STATE \hspace{3mm}  send $\langle \textsc{GetReq} \ k, GST_c\rangle$  to server
\STATE \hspace{3mm}  receive $\langle \textsc{GetReply} \ v, ut, gst \rangle$
\STATE \hspace{3mm}   $DT_c \leftarrow max(DT_c,ut)$
\STATE \hspace{3mm}  $GST_c \leftarrow max(GST_c,gst)$
\RETURN $v$

\STATE \vspace{5mm} \textbf{PUT} (key $k$, value $v$)
\STATE \hspace{3mm} send $\langle \textsc{PutReq} \ k,v,DT_c \rangle$ to server
\STATE \hspace{3mm} receive $\langle \textsc{PutReply} \ ut \rangle$ 
\STATE \hspace{3mm} $DT_c \leftarrow max(DT_c,ut)$

\end{algorithmic}
}
\end{algorithm}

\iffalse 
%Alogithm of GentleRain with HLC
\begin{algorithm} 
{
\caption{Client operations at client $c$ (These functions are identical to that of \cite{??} except that GST, gst, DT are hybrid logical clocks instead of physical clocks) }
\label{alg:client}
\begin{algorithmic} [1]

%\STATE // 
%\STATE 
\STATE \textbf{GET} (key $k$) %\COMMENT{ }

\STATE \hspace{3mm}  send $\langle \textsc{GetReq} \ k, GST_c\rangle$  to server
\STATE \hspace{3mm}  receive $\langle \textsc{GetReply} \ v, ut, gst \rangle$
\STATE \hspace{3mm}   $DT_c \leftarrow max(DT_c,ut)$
\STATE \hspace{3mm}  $GST_c \leftarrow max(GST_c,gst)$
\RETURN $v$

\STATE \vspace{5mm} \textbf{PUT} (key $k$, value $v$)
\STATE \hspace{3mm} send $\langle \textsc{PutReq} \ k,v,DT_c \rangle$ to server
\STATE \hspace{3mm} receive $\langle \textsc{PutReply} \ ut \rangle$ 
\STATE \hspace{3mm} $DT_c \leftarrow max(DT_c,ut)$

\end{algorithmic}
}
\end{algorithm}
\fi

When a client wants to write the value of an item, it sends a $\textsc{PutReq}$ message to the server maintaining the item. In addition to the key and value of the item, the client also piggybacks the value of its $DT_c$ to the message. The sever uses $DT_c$ to assign a timestampt to new version that is higher than $DT_c$. This is required to satisfied the condition $I1$ defined in Section \ref{??}. Client then wait to receive the reply from the server. In the $\textsc{PutReply}$ message, the server sends timestamp assigned to the new version. The client use this value to update it $DT_c$ as shown in Algorithm \ref{alg:client}. 

\subsection{Server Side}
In this section we focus on the server side of the protocol. Table \ref{??} shows variables that define the state for a server $p^m_n$. $PC^m_n$ and $HLC^m_n$ are the physical clock and the hybrid logical clock of partition $p^m_n$, respectively. $VV^m_n$ maintains the latest (HLC) timestamp received from other replicas. Specifically, $VV^m_n[k]$ is the latest timestamp received from server $p^k_n$. $LST^m_n$ is minimum timestamp that $p^m_n$ has received from its peers in other data centers. In other words, $LST^m_n$ maintains the minimum value in $VV^m_n$. Servers share their $LST^m_n$ with each other, and compute GST. $GST^m_n$ is the GST computed in server $p^m_n$. $LRT^m_n$ is the value of physical clock at the time of the most recent message to other replicas by server $p^m_n$.

\begin{center}
\begin{table} [h]
\caption{Variables maintained by server $p^m_n$}
\begin{tabular}{ |l|l|l| } 
\hline
\textbf{Symbol} & \textbf{Definition} \\
\hline
$PC^m_n$ &  current physical clock time at $p^m_n$\\ 
$HLC^m_n$ &  current hybrid logical clock time at $p^m_n$\\ 
$VV^m_n$ & version vector of $p^m_n$ , with $M$ elements \\ 
$LST^m_n$ & local stable time at $p^m_n$ \\ 
$GST^m_n$ & global stable time at $p^m_n$ \\ 
$LRT^m_n$ & Last (physical) time that server $p^m_n$ sent replicate or heartbeat message\\ 
\hline
\end{tabular}
\end{table}
\end{center}

Algorithm \ref{??} and Algorithm \ref{??} show the server side operation of MSU-DB. Upon receiving a GET request ($\textsc{GetReq}$), the server first update its GST by the GST value piggybacked to the GET request by the client. Next, server find the latest version of the item $d$  with the requested key that either is written in the local data center, or has the timestamp smaller than the $GST^m_n$. The server return the found value, $d.v$ together with it update time $d.ut$.


Upon receiving a PUT request by server $p^m_n$, the server first update it HLC by calling function $updateHLCforPut$. This function update the $HLC^m_n$ by the algorithm of the HLC, and uses the dependency timestamp ($dt$) sent by the PUT request. After updating the $HLC^m_n$, the server update its own entry in $VV^m_n$ with the $HLC^m_n$. Next, the server creates a new version for the item specified by the client and uses the current $HLC^m_n$ value for its timestamp. Then, it sends back the assigned timestamp to the client. 

Upon creating new version for an item in one data center, we should replicate the new version to other replicas in other data center. The server, also update it $LRT^m_n$ to keep track of the time of its most recent message to other replicas.  
Upon receiving a replicate message from server $p^k_n$, the receving server adds the new item to the version chain of key $d.k$. The server also updates the entry for server $p^k_n$ in its version vector. Thus, it sets $VV^m_n[k]$ to $d.ut$. 

\begin{algorithm} [t]
{
\caption{Server operations at server $p^m_n$ (part 1)}
\label{alg:server1}
\begin{algorithmic} [1]
\STATE \textbf{Upon} receive $\langle \textsc{GetReq} \ k, gst \rangle$
\STATE \hspace{3mm} $GST^m_n \leftarrow max(GST^m_n, gst)$
\STATE \hspace{3mm}  obtain latest version $d$ from version chain of key $k$ s.t. $d.sr = m or d.ut \leq GST^m_n$
\STATE \hspace{3mm} send $\langle\textsc{GetReply} \  d.v, d.ut, GST^m_n\rangle$ to client


\STATE \vspace{5mm} \textbf{Upon}  receive $\langle \textsc{PutReq} \ k, v, dt \rangle$
\STATE \hspace{3mm}  $updateHCLforPut(dt)$
\STATE \hspace{3mm}  $VV^m_n  [m] \leftarrow HLC^m_n$
\STATE \hspace{3mm}  Create new item $d$
\STATE \hspace{3mm}  $d.k \leftarrow k$ 
\STATE \hspace{3mm}  $d.v \leftarrow v$
\STATE \hspace{3mm}  $d.ut \leftarrow HLC^m_n$
\STATE \hspace{3mm}  $d.sr \leftarrow m$ 
\STATE \hspace{3mm}  insert $d$ to version chain of $k$
\STATE \hspace{3mm}  send $\langle PutReply, d.ut \rangle$ to client

\STATE \vspace{5mm} \textbf{Upon}   new version $d$ created
\STATE \hspace{3mm}  \textbf{for} each server $p^k_n, k \in \{0 \ldots M-1\}, k \neq m$ \textbf{do}
\STATE \hspace{6mm}  send $\langle \textsc{Replicate} \ d \rangle$ to $p^k_n$
\STATE \hspace{3mm}  $LRT^m_n \leftarrow PC^m_n$

\STATE \vspace{5mm} \textbf{Upon}  receive $\langle \textsc{Replicate} \  d \rangle$ from $p^k_n$
\STATE \hspace{3mm}  insert $d$ to version chain of key $d.k$
\STATE \hspace{3mm} $VV^m_n  [k] \leftarrow d.ut$



\STATE \vspace{5mm} \textbf{UpdateHLCforPut ($dt$)}
\STATE \hspace{3mm} $l’ = HLC^m_n.l$
\STATE \hspace{3mm} $HLC^m_n.l = max (HLC^m_n.l, PC^m_n, dt.l)$
\STATE \hspace{3mm} \textbf{if} $(HLC^m_n.l = l' = dt.l) \ \ HLC^m_n.c \leftarrow max(HLC^m_n.c ,dt.c)+1$
\STATE \hspace{3mm} \textbf{else if} $(HLC^m_n.l = l') \  \ HLC^m_n.c \leftarrow HLC^m_n.c + 1$
\STATE \hspace{3mm} \textbf{else if} $(HLC^m_n.l = l) \  \ HLC^m_n.c \leftarrow dt.c + 1$
\STATE \hspace{3mm} \textbf{else} $HLC^m_n.c = 0$


\end{algorithmic}
}
\end{algorithm}


A server sends heartbeat messages to its peers in other data centers if it has not send any replicate message to its peers for certain time $\Delta$. Thus, every $\Delta$ time, if $LRT^m_n + \Delta$ is less than or equal to current physical time, $PC^m_n$, the server decides to send heartbeat message. Before sending the heartbeat message, the server first update it $HLC^m_n$ by calling function $udpateHCL$. This function update $HLC^m_n$ as described in Section \ref{??}. The server, next, update its own entry in $VV^m_n$ and $LRT^m_n$. Then, sends heartbeat messages to its peers in other data centers. Upon receiving a heartbeat message from server $p^k_n$, server $p^m_n$ sets $VV^m_n[k]$ to HLC time received by the heartbeat message.

Every $\theta$ time, servers compute their LSTs and communicate LSTs to compute GST. The communicating LSTs and computing GST is done by a tree construction as in GentleRain \cite{??}.


\begin{algorithm} 
{
\caption{Server operations at server $p^m_n$ (part 2)}
\label{alg:server2}
\begin{algorithmic} [1]



\STATE \vspace{5mm} \textbf{Upon} every $\Delta$ time
\STATE \hspace{3mm} $ct \leftarrow PC^m_n$
\STATE \hspace{3mm} \textbf{if} $ct \geq LRT^m_n + \Delta$ 
\STATE \hspace{6mm}  $updateHCL()$
\STATE \hspace{6mm}  $VV^m_n  [m] \leftarrow HLC^m_n$
\STATE \hspace{6mm}  $LRT^m_n \leftarrow ct$
 \STATE \hspace{6mm}  \textbf{for} each server $p^k_n, k \in \{0 \ldots M-1\}, k \neq m$ \textbf{do}
\STATE \hspace{9mm}  send $\langle \textsc{Heartbeat} \ HLC^m_n \rangle$ to $p^k_n$


\STATE \vspace{5mm} \textbf{Upon}  receive $\langle \textsc{Heartbeat} \ hlc \rangle$ from $p^k_n$
\STATE \hspace{3mm}  $VV^m_n  [k] \leftarrow hlc$


\STATE \vspace{5mm} \textbf{Upon}  every $\theta$ time
\STATE \hspace{3mm} $LST^m_n \leftarrow min(VV^m_n)$
\STATE \hspace{3mm} $GST^m_n \leftarrow min(\{ LST^m_k | 0 \leq k \leq N-1 \} )$



\STATE \vspace{5mm} \textbf{UpdateHLC ()}
\STATE \hspace{3mm} $l’ = HLC^m_n.l$
\STATE \hspace{3mm} $HLC^m_n.l = max(HLC^m_n.l, PC^m_n)$
\STATE \hspace{3mm} \textbf{if} $(HLC^m_n.l = l’)\ $ $HLC^m_n.c \leftarrow HLC^m_n.c + 1$
\STATE \hspace{3mm} \textbf{else} $HLC^m_n.c \leftarrow 0$

\end{algorithmic}
}
\end{algorithm}


==> related.tex <==
\section{Related Work}
\label{sec:related}
\iffalse
{\bf Consistency and Availability}.  \ 
Strong consistency (a.k.a. linearizability) defines a total ordering on all operations on the system. Causal consistency gives a partial order over operations so the clients see operations in an order imposed by the causality relation~\cite{lamport}.

The CAP theorem~\cite{cap} states that a distributed system cannot maintain strong consistency and availability in the presence of partitions. Refining this result, the CAC theorem~\cite{mahajan2011} states that in an asynchronous model with omission-failures and unreliable networks, no consistency stronger than real-time causal consistency (RTC) can be provided in an always-available, one-way convergent system and RTC can be provided in an always-available, one-way convergent system. An always available system allows reads and writes to complete regardless of lost messages (i.e., no operation can block indefinitely or return an error signifying unavailability of data), and a one-way convergent system guarantees that if node $p$ can receive from node $q$, then eventually $p$'s state reflects updates known to $q$. MSU-DB is able to provide causal consistency and availability in a one-way convergent system as in COPS~\cite{COPS}.

{\bf Strong consistency}. \
ABD algorithm achieves strong consistency and atomic updates.

{\bf COPS}. \ 
%http://muratbuffalo.blogspot.com/2012/09/dont-settle-for-eventual-scalable.html
COPS~\cite{COPS} is a distributed storage system that provides causal+ consistency across WAN. In COPS, a put operation for a record is: i) translated to put-after-dependencies based on the dependencies seen at this site; ii) queued for asynchronous replication to other sites; iii) returned success to the client at this point (early reply); and iv) asynchronously replicated to other sites. Each operation maintains dependencies for operations, which are checked at each datacenter before replication and when they are satisfied the value is updated there.


GentleRain and MSU-DB provide causal consistency more efficiently than COPS, because they do not need to maintain, exchange, and check dependency lists, which can grow very large in size. 
\fi

